Invariant manifolds and the long-time asymptotics of the Navier-Stokes and vorticity equations on R^2

We construct finite-dimensional invariant manifolds in the phase space of the Navier-Stokes equation on R^2 and show that these manifolds control the long-time behavior of the solutions. This gives geometric insight into the existing results on the asymptotics of such solutions and also allows one to extend those results in a number of ways.

==> Fig1.tex <==
% height 5.5 cm
% width 11.0 cm	
\smash{\hbox{
\point	8.60	3.05 	{$\Re(\lambda)$}
\point	7.40	5.00 	{$\Im(\lambda)$}
\point	5.20	4.50 	{$\textstyle \frac{m}{2}-\frac{1}{2}$}
\point	4.70	2.20 	{$-1$}
\point	5.80	2.20 	{$\textstyle -\frac{1}{2}$}
\point  7.00    2.20    {$0$}
\point	1.80	1.50 	{$\sigma_c(\cL)$}
}}



==> Fig2.tex <==
% height 5.5 cm
% width 11.0 cm	
\smash{\hbox{
\point	9.00	3.55 	{$E_c$}
\point	4.55	7.10 	{$E_s$}
\point	6.65	3.60 	{$w$}
\point	6.90	6.00 	{$M_w$}
\point	8.60	2.60 	{$W_c$}
\point	5.20	6.00 	{$M_0$}
\point	4.50	3.45 	{$0$}
}}



==> Fig3.tex <==
% height 5.5 cm
% width 11.0 cm	
\smash{\hbox{
\point	6.65	3.65 	{$W_c$}
\point	7.40	2.35 	{$E_c$}
\point	3.75	6.15 	{$E_s$}
\point	4.00	5.00 	{$W_s$}
}}


